Comparison of Unscented Kalman Filter Design for Agricultural Anaerobic Digestion Model

Dynamic operation of biological processes, such as anaerobic digestion (AD), requires reliable process monitoring to guarantee stable operating conditions at all times. Unscented Kalman filters (UKF) are an established tool for nonlinear state estimation, and there exist numerous variants of UKF implementations, treating state constraints, improvements of numerical performance and different noise cases. So far, however, a unified comparison of proposed methods emphasizing the algorithmic details is lacking. The present study thus examines multiple unconstrained and constrained UKF variants, addresses aspects crucial for direct implementation and applies them to a simplified AD model. The constrained UKF considering additive noise delivered the most accurate state estimations. The long run time of the underlying optimization could be vastly reduced through pre-calculated gradients and Hessian of the associated cost function, as well as by reformulation of the cost function as a quadratic program. However, unconstrained UKF variants showed lower run times at competitive estimation accuracy. This study provides useful advice to practitioners working with nonlinear Kalman filters by paying close attention to algorithmic details and modifications crucial for successful implementation.

==> Input/Abstract.tex <==
\begin{abstract}
Dynamic operation of biological processes, such as anaerobic digestion (AD), requires reliable process monitoring to guarantee stable operating conditions at all times. Unscented Kalman filters (UKF) are an established tool for nonlinear state estimation, and there exist numerous variants of UKF implementations, treating state constraints, improvements of numerical performance and different noise scenarios. So far, however, a unified comparison of proposed methods emphasizing the algorithmic details is lacking. The present study thus examines multiple unconstrained and constrained UKF variants, addresses aspects crucial for direct implementation and applies them to a simplified AD model. The constrained UKF considering additive noise delivered the most accurate state estimations. The long run time of the underlying optimization could be vastly reduced through pre-calculated gradients and Hessian of the associated cost function, as well as by reformulation of the cost function as a quadratic program. However, unconstrained UKF variants showed lower run times and competitive estimation accuracy. This study provides useful advice to practitioners working with nonlinear Kalman filters by paying close attention to algorithmic details and modifications crucial for successful implementation. 

%{\color{blue} The complexity of biogas plant processes, determined by nonlinear dynamics and constraints, poses a difficult challenge for state estimation and control. Ensuring positive concentration values of substrates (and states) further accentuates the necessity for sophisticated nonlinear estimation methods based on constraint optimization.
% (Recent developments have introduced simplified versions of the Anaerobic Digestions Model No.1 R4-(ADM1-R4) that hold promise for nonlinear model-based state estimation and process control in full-scale agricultural biogas plants.)n This study investigates various nonlinear state estimation techniques applied to the anaerobic digestion model in simulation studies that encompass real experimental uncertainties. State estimation methods, including the Unscented Kalman Filter, as well as constraint-based approaches, were rigorously examined and tested. Furthermore, to improve efficiency of constrained optimization based Unscented Kalman filter, both the speed and function evaluation were optimized by leveraging pre-calculated gradients and Hessians. The findings from this research contribute to the advancement of nonlinear state estimation methodologies within the domain of anaerobic digestion, offering valuable insights for improved process monitoring, control and optimization of real-world biogas-plant applications.}
\end{abstract}

\begin{IEEEkeywords}
	Process monitoring, nonlinear state estimation, sigma point Kalman filter, biogas technology, ADM1%, 
\end{IEEEkeywords}

% Stichwörter: 

% 1. nonlinear process monitoring 
% demand-driven operation of biogas plants
% stable plant operation

% 2. among the manifold UKF implementations, which one is most appropriate for AD model? 
% 3. various implementation details of the algorithms not precisely specified 

% 4. unconstrained and constrained UKF variants, some numerical improvements and apply to reduces model of the AD process

% 5. The constrained UKF with additive noise provided best accuracy, while unconstrained alternatives show lower run times and comparable estimation accuracy.

% 6. algorithmic modifications and emphasis on crucial details provide advice to practitioners working with KF. 
